Preventing Cheating in Hands-on Lab Assignments

Networking, operating systems, and cybersecurity skills are exercised best in an authentic environment. Students work with real systems and tools in a lab environment and complete assigned tasks. Since all students typically receive the same assignment, they can consult their approach and progress with an instructor, a tutoring system, or their peers. They may also search for information on the Internet. Having the same assignment for all students in class is standard practice efficient for learning and developing skills. However, it is prone to cheating when used in a summative assessment such as graded homework, a mid-term test, or a final exam. Students can easily share and submit correct answers without completing the assignment. In this paper, we discuss methods for automatic problem generation for hands-on tasks completed in a computer lab environment. Using this approach, each student receives personalized tasks. We developed software for generating and submitting these personalized tasks and conducted a case study. The software was used for creating and grading a homework assignment in an introductory security course enrolled by 207 students. The software revealed seven cases of suspicious submissions, which may constitute cheating. In addition, students and instructors welcomed the personalized assignments. Instructors commented that this approach scales well for large classes. Students rarely encountered issues while running their personalized lab environment. Finally, we have released the open-source software to enable other educators to use it in their courses and learning environments.

==> boxplot-chains.tex <==
%%% Puvodni cast psana stylem Benefits and Pitfalls paperu
\begin{comment}
In this part, we focused on the suspicious speed of passing the consecutive challenges. We estimated the technically minimal possible time to solve the challenge by an expert participant who immediately enter the answer. \Cref{fig:chains} depicts the time between submission of correct answer and the submission of correct answer in the preceding challenge in the same chain. 

\begin{figure}[h!]
    \centering
    % boxplotdata.dat form -> index median box_top box_bottom whisker_top whisker_bottom
    \scalebox{0.80}{ % \scalebox{<h-scale>}[<v-scale>]{<content>} 
   %  \small
        \begin{tikzpicture}%[fixed ratio=16:9]
            \begin{axis} [
                ymode=log,
                xtick={1,2,3,4,5,6,7,8},
                xticklabels={A1,A2,A3,A4,S1,S2,T1,T2},
                ytick={30, 60, 120, 300, 600, 1800, 3600,14400, 86400},
                yticklabels={30s,1m,2m,5m,10m,30m,1h,4h,1d},
                %yticklabels={Not at all, Slightly, Moderately, Much, Very much},
            ]
                \addplot [box plot median] table [opacity=0.5]{boxplotsubmissionspeed.dat};
                \addplot [box plot box] table {boxplotsubmissionspeed.dat};
                \addplot [box plot top whisker] table {boxplotsubmissionspeed.dat};
                \addplot [box plot bottom whisker] table {boxplotsubmissionspeed.dat};
                \draw [green,ultra thick] (0.75,3.5) -- (1.25,3.5); % task 1
                \draw [green,ultra thick] (1.75,1) -- (2.25,1); % task 2
                \draw [green,ultra thick] (2.75,45) -- (3.25,45); % task 3
                \draw [green,ultra thick] (3.75,1) -- (4.25,1); % task 4
                \draw [green,ultra thick] (4.75,46) -- (5.25,46); % task 5
                \draw [green,ultra thick] (5.75,33) -- (6.25,33); % task 6
                \draw [green,ultra thick] (6.75,16) -- (7.25,16); % task 7
                \draw [green,ultra thick] (7.75,78) -- (8.25,78); % task 8
                
                %% instructors time
                %\draw [blue,ultra thick] (0.75,6) -- (1.25,6); % task 1
                %\draw [blue,ultra thick] (1.75,120) -- (2.25,120); % task 2
                %\draw [blue,ultra thick] (3.00,45) -- (3.25,45); % task 3 --> same for all
                %\draw [blue,ultra thick] (3.75,240) -- (4.25,240); % task 4
                %\draw [blue,ultra thick] (5.00,46) -- (5.25,46); % task 5  --> same for all
                %\draw [blue,ultra thick] (6.00,33) -- (6.25,33); % task 6  --> same for all
                %\draw [blue,ultra thick] (7.00,16) -- (7.25,16); % task 7  --> same for all
                %\draw [blue,ultra thick] (8.00,78) -- (8.25,78); % task 8  --> same for all
            \end{axis}
        \end{tikzpicture}
    }
    \caption{Time between submission of correct answer of two consecutive challenges.}%nadpis prevzat z Benefits and Pitfalls paperu
    \label{fig:chains}
\end{figure}
\end{comment}
